Evolution of Non-Terrestrial Networks From 5G to 6G: A Survey

Non-terrestrial networks (NTNs) traditionally have certain limited applications. However, the recent technological advancements and manufacturing cost reduction opened up myriad applications of NTNs for 5G and beyond networks, especially when integrated into terrestrial networks (TNs). This article comprehensively surveys the evolution of NTNs highlighting their relevance to 5G networks and essentially, how it will play a pivotal role in the development of 6G ecosystem. We discuss important features of NTNs integration into TNs and the synergies by delving into the new range of services and use cases, various architectures, technological enablers, and higher layer aspects pertinent to NTNs integration. Moreover, we review the corresponding challenges arising from the technical peculiarities and the new approaches being adopted to develop efficient integrated ground-air-space (GAS) networks. Our survey further includes the major progress and outcomes from academic research as well as industrial efforts representing the main industrial trends, field trials, and prototyping towards the 6G networks.

==> 5G.tex <==
 \section{Integration of NTN into 5G NR \\ \green{[TBD]}  \\ (max 3 pages text)}\label{sec:NTN5G}

\subsection{Satellite in 5G NR}
References: \cite{3GPP38811,3GPP22822,3GPP38821,lin20195g,rinaldi2020non,guidotti2019architectures}
    \begin{itemize}
        % \item Use cases based on service enablers \cite[Table 4.2.1]{3GPP38811}
        % We speak about use cases for 5G service enablers, i.g.
        % \begin{itemize}
        %     \item eMBB
        %     \item mMTC
        % \end{itemize}
        \item Use cases based on services \cite{3GPP38821,3GPP22822, rinaldi2020non}
        % From a different angle we could also speak about use cases for enabling the followings:
        % \begin{itemize}
        %     \item Service continuity
        %     \item Service ubiquity
        %     \item Service scalability 
        % \end{itemize}
        \item Architecture \cite{3GPP22822, rinaldi2020non, bi2019software}
        \item Requirements and considerations \cite{3GPP38811,3GPP38821, 3GPP22125, 3GPP22822}
        % \item Channel modeling
        % \begin{itemize}
        %     \item Outside of 3GPP: ITU-R P.681, ITU-R P.618
        %     \item 3GPP modeling \cite{3GPP38811}
        %     \item Tractable modeling for theoretical study \cite{fang20205g,al2020modeling}
        % \end{itemize}
        \item NR Deployment and challenges to support NTN \cite{guidotti2019architectures, rinaldi2020non, 3GPP38821}
        \item Performance evaluation \cite{fang20205g,okati2020downlink,al2021analytical,zeydan2019impact}
        \item High Altitude Platform Stations as IMT Base Stations \cite{3GPP38821,euler2020primer,dao2021survey,kurt2021vision} 
        \item Inter-satellite connectivity \cite{leyva2020inter,babich2019nanosatellite,leyva2020constellations}  
    \end{itemize}
 
\subsubsection{Use cases}

While 5G NR has been designed as a terrestrial network, 3GPP has ongoing efforts on integrating NTN into 5G and beyond 5G networks. Because NTN showcase a reduced vulnerability to physical attacks and natural disasters and can provide wide spread coverage, three main categories for the use cases are defined by 3GPP \cite{3GPP38821, 3GPP22822}. First of all, service continuity, the deployment of the terrestrial network could be centered around urban areas, resulting in areas with no coverage. NTN could provide services to UE's travelling into these no-coverage zones. Secondly, service ubiquity, in the case that the terrestrial network is not available due to a disaster or economic reasons, for example on a large field equipped with IoT nodes. In this case NTN could provide access to the users in these areas that want to access 5G services. Lastly, scalablity, NTN can provide efficient broadcasting services, allowing streaming content to large areas and offloading popular content to the network edge. These roles fit mainly within the 5G eMBB and mMTC use cases. On the other hand, the large propagation delays of satellites makes NTN less interesting for the URLLC use case for obvious reasons \mahdi{how about UAVs for URLLC? NTN includes UAV-based networks too.}. \cite{rinaldi2020non} provides an overview of the 3GPP NTN features, uncovering their potential to satisfy consumer expectations in 5G networks. \mahdi{Repetitive! This paragraph should be integrated with the content in the Preliminaries section.}

\mahdi{1. NTN for continuity, ubiquity, and scalability, 2. NTN for eMBB, URLLC, and mMTC}

\subsubsection{Architecture}
In the context of 5G NR, the following system elements are generally considered part of an NTN\cite{3GPP22822, rinaldi2020non}. An NTN Terminal is a ground terminal directly connected to the satellite system, can be either a UE or specific termal such as a gNB. A service link representing the link between the UE and the airborne equipment. The user can be simultaneously connected to a terrestrial platform. Two types of payload on the airborn platform are considered. Either the airborn platform can support either a bent pipe payload, basically relaying the signals from a terrestrial gateway in a transparent manner or it can support a regenerative payload, which decodes/demodulates and codes/modulates the signal from a terrestrial gateway, effectively operating as a (partial) gNB. Inter satellite links are supported in case of a constellation of satellites and a regenerative payload. A gateway connects the aerial platform to the core network. Feeder links, are defined as the radio links between gateway and space platform. An architecture that integrates space and terrestrial components using software defined networking is presented in \cite{bi2019software}. \mahdi{Repetitive! --> Preliminaries section.}

 
% \subsubsection{Requirements and considerations}

% When it comes to integrating NTN in 5G NR networks, several additional functionalities and requirements of the 5G network have been proposed by the 3GPP consortium \cite{3GPP38811,3GPP38821, 3GPP22125, 3GPP22822}. The network should be able to support roaming between terrestrial and satellite network, performing vertical handovers when necessary. The UE can be in full control when to use the terrestrial network and when to use the satellite network. Two types of satellite and Aerial networks are considered. One providing broadband access network by serving Very Small Aperture Terminals fixed to moving platform operating in frequency bands above $6~GHz$, in the so called $K_a$ band. The other type providing a narrow or wide band access network to terminals equipped with omni directional antennas, operating in frequency  bands below $6~GHz$ in the so called S band.


\subsubsection{NR Deployment and challenges to support NTN}

Several challenges are raised when introducing NTN in 5G NR networks\cite{guidotti2019architectures}. First of all, satellite platforms are not capable of serving users indoor, only lower altitude platforms such as HAP and UAVs are suited for this scenario\cite{rinaldi2020non}. Next, users will experiences different propagation delays in different regions of the cell due to the large coverage areas. This will affect the initial access and synchronization of users at the cell center and cell edge. Similarly, longer propagation delay could impact protocol layers in terms of retransmissions and response time and large propagation delays could result in outdated CQI measurements. Furthermore, large frequency shifts due to Doppler should be considered when determining the Subcarrier Spacing of the OFDM signal. Moving cells will cause handovers for static users, however these can be anticipated with satellite trajectory models. The addition of the targeted new spectrum, S band and $K_a$ band, requires a review of the channel numbering, especially to support the above $6~GHz$ bands the 5G NR radio interface should be adopted to support FDD operation in Frequency Range 2. The reference signals used to monitor signal strengths for example should be adapted to take into account Doppler and possible specific multipath effects \cite{3GPP38821}. \mahdi{Move to Preliminaries}

\subsubsection{Performance evaluation}

To evaluate the integration of NTN in 5G NR, several works have attempted at modeling the performance of an 5G NR NTN. For example, \cite{fang20205g} provides insight in the operation of NTN by proposing three cooperative models to understand hybrid satellite-terrestrial networks models, and evaluating the state-of-the-art technologies for each model. On the other hand, \cite{okati2020downlink} presents a model based on a stochastic approach to analyse downlink and rate of low orbit satellite networks. Similarly, \cite{al2021analytical} presents a framework based on stochastic geometry to evaluate dense satellite networks by deriving interference statistics and coverage probability. Authors of \cite{zeydan2019impact} provide an experimental evaluation of NTN 5G networks, where they compare satellite and terrestrial based backhaul networks.\mahdi{...}

% \subsubsection{High Altitude Platform Stations as IMT Base Stations}
  
% Release 17 includes support of High Altitude Platform Stations as IMT Base Stations (HIBS) \cite{3GPP38821}, which can be deployed to expand the availability of broadband in remote regions. Due to recent development in solar panel efficiency, battery energy density, lightweight composite materials, autonomous avionics and antennas these type of platforms are becoming more and more viable. An overview of the current status on development of HIBS is presented in \cite{euler2020primer}. As well as some preliminary system level simulation results to shed some light on the performance of HIBS. Authors of \cite{dao2021survey} provide an overview on recent literature on aerial access networks within 5G. To meet the 5G standards requirements of coverage and capacity \cite{kurt2021vision} introduces HAPS-Mounted Super Macro Basestation (HAPS-SMBS) as a powerful tool to enhance connectivity due to their large coverage footprint, high computational power and good LOS conditions. Several use-cases are presented such as delivering IoT services, supporting aerial networks and back-hauling isolated BSs followed by a discussion on the general requirements and the feasibility of the deployments of these use cases.

\subsubsection{Inter-Satellite Connectivity}
 A satellite might not always be connected to the core network, for example when no gateway can be reached, this could impact latency of the link. To solve this, satellites can be connected with other satellites and form constellations through Inter-Satellite Links (ISL), reaching a gateway via Inter-Satellite hops. The role of these constellations within 5G is discussed in \cite{leyva2020constellations}. The impact of ISL on latency of the link can be found in \cite{babich2019nanosatellite}. A detailed analysis of the connectivity between LEO satellites in different orbital planes can be found in \cite{leyva2020inter}, evaluating achievable data rates, impact of interference and propagation delays. A framework and the corresponding algorithms are proposed for the dynamic establishment of the inter-plane ISLs. \mahdi{move to Preliminaries.}
%\red{can be extended to inter HAPs links?HAPS constellations\cite{kurt2021vision}} 


\subsection*{Satellite Integration in mmWave}
Among all discussed NTN technologies, the use of satellites utilizing mmWave frequencies promises the largest intrinsic high capacity capabilities, while simultaneously supporting global coverage. Thus, 3GPP's release 16 envisions satellite links to offer broadband services over mmWave frequencies because of the availability of huge bandwidths and highly directive/spatial resolution \cite{3GPP38821}. However, these mmWave signals undergo severe Doppler shifts and several stages of attenuation as presented by \cite{giordani2020satellite}. To counter these large losses, highly directive antennas are used. Terrestrial terminal are equipped with Very Small Aperture Terminal (VSAT) while the satellites are equipped with reconfigurable phased antenna arrays supporting highly directive beamforming resulting in antenna gains of $50~dB$ and more. At high frequencies antenna elements become significantly smaller allowing the creation of very large antenna arrays, which can support these very directive beams but can also support more advanced technologies such as multibeam architectures \cite{giordani2020non}. In \cite{babich2019nanosatellite} a complete network architecture for an integrated nSAT-5G mmWave system is envisioned, where a constellation of nSATS communicating through mmWave links operate as gateways between several isolated terrestrial gNB's. A detailed architecture is presented and a comprehensive analysis of the system is performed by implementing the system in NS3.
% References: \cite{babich2019nanosatellite,giordani2020non,giordani2020satellite}
% \begin{itemize}
%     \item Scenarios
%     \item Modeling and performance analysis
% \end{itemize}    
% \subsubsection*{Scenarios}
% Within 5G NR, several scenarios of satellites operating mmWave in can be considered.
% \begin{itemize}
%   \item{\textbf{Backhauling:}} 
%   A mmWave satellite can provide broadband connectivity between the core network and a cell in un-served areas. The isolated cell is equiped with a VSAT and implements a 
%   \item{\textbf{Relaying and broadcasting:}} 
%   \item{\textbf{In-motion terminals:}} 
%  \end{itemize}

\subsubsection*{Modeling and performance analysis}
Several simulations performed by \cite{giordani2020satellite} demonstrate the potential of high capacity of highly-directional satellite mmWave communications to over wide geographical coverage. In \cite{giordani2020non} the performance was evaluated of a scenario where satellites use mmWave frequencies to provide broadband connectivity to terrestrial mobile UEs. They show that Shannon capacity decreases when increasing altitude going from LEO to GEO, nonetheless gigabits-per-seconds can be achieved mainly due to the large antenna gains of the large antenna arrays creating narrow beams. For GEO satellites these pencil beams are feasible due to the relative stationary to earths surface.


\subsection{UAV in 5G NR}
\begin{itemize}
       \item Use cases \cite{mozaffari_2019, mozaffari2019tutorial, zeng2019accessing}
        \item UAV as user \cite{colpaert2018aerial,vinogradov2019tutorial,vinogradov2019uav, 3GPP36777,3GPP22125}
        \item UAV as network node \cite{cicek2019UAV,li2018uav,mozaffari2019tutorial,bekkouche2020service}
    \end{itemize}
    
% \cite{mozaffari_2019, mozaffari2019tutorial, zeng2019accessing}
\subsubsection*{Use cases}
Past years, the UAV application market has been growing drastically. Many industries see UAVs as business opportunity for the next decade. A important requirement to the potential success of these UAVs is their connectivity. Integration into the 5G network has been proposed to allow for UAVs to operate in a virtual unlimited operation range. Utilizing the upcoming 5G cellular network is a cost efficient use of of infrastructure, and could push to further speed up the deployment of 5G.
Authors of \cite{zeng2019accessing} provides a tutorial overview of the advances on integrating UAVs into the fifth generation cellular network. They raise the main problems of cellular connected UAVs, including LOS dominant UAV-ground channels, strong aerial-terrestrial network interference and the constraints in terms of size, weight and power. The work \cite{mozaffari_2019} introduces the concept of a 3D cellular network and analytical methods are used to characterise such 3D wireless networks. \cite{mozaffari2019tutorial} dives deeper into cellular connected UAVs and explores the challenges of channel modeling, performance analysis and 3D deployment with representative results. They also give an overview of the tools available to further address the UAV problems. Two distinct cases are distinguished: on one hand there is the UAV operating as a user and utilising the network as a means to provide many different services. On the other hand there is the UAV that is part of the network infrastructure, further extending the 5G network.
\subsubsection*{UAVs as a user}
% \cite{3GPP36777, mozaffari2019tutorial, zeng2019accessing}
This scenario appeals to most the companies as it could benefit many different industries, such as logistics, maintenance, surveillance, agriculture and so on. To support these types of services, the UAV needs reliable and low-latency communication to operate the drones remotely, while simultaneously supporting the potential large data-rates that these applications could imply. One of the largest challenges in this scenario is the fact that cellular networks are mainly designed for ground users\cite{ colpaert2018aerial, vinogradov2019tutorial}. Mobility, operations and traffic characteristics are significantly different from ground users. Firstly, aerial users experience different wireless channel properties and LOS links to the ground network will cause significant levels of interference. Secondly, due to their highly mobility, UAVs will be more dynamic than ground users. Finally, due to the UAVs being battery powered, on-board energy becomes one of the constraints, to solve this researchers are looking into deploying UAVs on demand. Another issue pointed out by \cite{vinogradov2019uav} is the interference caused by UAVs to existing satellite applications. While 3GPP has made efforts into supporting UAVs in the future \cite{3GPP36777,3GPP22125}, it still remains to be seen how effective cellular-connected UAVs will be.
\subsubsection*{UAV as network node}
A popular researched topic in the UAV communications field is the performance of a network that has one or more UAVs deployed as part of its infrastructure. In this context, many works describe the ideal positioning of these aerial basestations \cite{cicek2019UAV}, serving users in disaster scenarios where the existing network broke down, or serving users at places where the network is overloaded. In \cite{li2018uav} an extensive review of several 5G techniques based on UAV platforms is given. The tutorial of \cite{mozaffari2019tutorial} compares UAV basestations to terrestrial basestations and discusses the key applications of UAV-mounted aerial basestations in 5G. The work of \cite{bekkouche2020service} provides an overview of different UAV deployment options and then analyzes the required enhancements to the network architecture.



% \begin{itemize}
%     \item{\textbf{UAV as UE:}} 
%     UAVs operating within 3D highways for fast and efficient service deliveries. optimal trajectory design, limited battery
%     \item{\textbf{UAV as gNb:}} 
%     UAVS operating as basestation in disaster scenarios.
%     UAVS to offload traffic from congested areas
% \end{itemize}
%     \begin{itemize}
%         \item Use cases and requirements
%         UAV as user
%         UAV as BS
%         % \item Review of the 3GPP work
%         \item Performance improvements
%         \begin{itemize}
%             \item URLLC [5G-Sky]
%             \item mmwave beam-forming, beam-tracking, and beam-selection \cite{kalamkar2020beam,meng20205g} \cite{song2020beam,zhang2019fast,yang2020performance}
%             To solve the interference issue, beamforming in the mmWave spectrum has been proposed. Assuming beamtracking.
%             \item swarm operation \cite{zhang2019fast,polese2020experimental,dabiri2020analytical}
%             To improve connectivity, UAVs can operate in swarms where only one relay UAV node is connected to the network. This to reduce downlink interference generated to the ground network. ISL equivalent for UAV?
%             % \item TBD
%         \end{itemize}
%         \item challenges of mmWave
%         A UAV will experience more handovers due to the LOS propagation conditions to most of the terrestrial base stations.
%         Beamtracking will be difficult.
%         Initial access.
%         Doppler shifts
%         their size, weight, and power (SWAP) constraints
        
            % \end{itemize}
%\end{itemize}

\subsection*{UAV Integration in mmWave}

\begin{itemize}
    \item Use cases \cite{xiao2016enabling,zhang2019research,zhang2019survey,xiao2020uav}
    \item UAV beamforming \cite{colpaert2018aerial,kalamkar2020beam,song2020beam,colpaert20203d}
\end{itemize}

\subsubsection*{Use cases}
To resolve the spectrum crunch crisis, 5G NR brings new spectrum opportunities in the form of mmWave. Although mmWave links suffer of large propagation losses and blockages by physical obstacles, the wide unoccupied bandwidths pose an attractive solution to reaching high data rates. Introducing mmWave communication to cellular connected UAVs has proven to have great potential \cite{xiao2016enabling}.
The work of \cite{zhang2019research} describes mmWave UAV channel characteristics and analyses the acquisition of UAV mmWave channels and precoder design. Both \cite{zhang2019survey} and \cite{xiao2020uav} present in their survey current achievements of 5G mmWave in UAV-assisted wireless networks and highlight three potential applications. First of all, aerial access, where a UAV provides access to the ground users by operating as an aerial BS. Secondly, UAVs can operate as an aerial relay, acting in a multi-hop fashion, providing indirect access to ground users. Finally, they mention aerial backhaul links to provide Gigabit data transmissions in a flexible manner. They both give an overview of the advantages and challenges of 5G mmWave communications for UAV-assisted networks.

\subsubsection*{UAV beamforming}
One of the advantages of using mmWave is the improved security and interference situation by using highly directive beamforming \cite{colpaert2018aerial}. However, it is also this beamforming that poses as one of the challenges, as beam misalignment becomes more prevalent with narrow beamwidth. Authors of \cite{kalamkar2020beam} provide a system-level stochastic geometry model to analyse the important aspects of mmWave beam management problems, while \cite{song2020beam} proposes a possible solution to perform consistent beam tracking from ground station to UAV in the form of a Kalman filter based tracking model. The fact that mmWave networks become more dense, will also pose problems in terms of handovers, as cell size will shrink dramatically in urban environments\cite{colpaert20203d}. 

% Another advantage is that the short wavelengths at mmWave frequencies result in all the RF hardware being physically small. Smaller mmWave equipped can easily be the payload of a drone and the small antenna aperture size allows us to fit antenna arrays with large numbers of antennas on UAVs. These large antenna arrays allow for flexible directive beamforming and even more advanced precoding techniques like Massive MIMO.

\subsection*{Inter-UAV communication}
\begin{itemize}
    \item Use cases \cite{vinogradov2019tutorial,vinogradov2020wireless,cherif20213d}
    \item Performance analysis \cite{dabiri2020analytical,yang2020performance,zhang2019fast,polese2020experimental,dabiri2020analytical,zhang2019survey,feng2018spectrum}
\end{itemize}
\subsubsection*{Use cases}
While it will be important for UAVs to be connected to the ground, it will be equally important for UAVs to be interconnected especially considering the predicted growth of UAVs in the sky\cite{vinogradov2019tutorial}. To avoid collisions sense and avoid techniques can be deployed which can be based either on broadcast signals, direct communication links or radar type applications \cite{vinogradov2020wireless}. To coordinate efficient airspace use collaborative UAV swarm techniques can be used, where drones can use specifically designated airspace for example in the form of drone highways \cite{cherif20213d}. Within NR, drones could use the available device-to-device communications to exchange messages between themselves.

\subsubsection*{Performance analysis}
In the context of UAV swarms, \cite{yang2020performance} formulates performance and fairness in the context of UAV swarms connected to cellular networks. \cite{zhang2019fast} on the other hand, presents an inter-UAV beam tracking scheme, capable of overcoming slight beam misalignment. An experimental analysis of the UAV-to-UAV mmWave channel is performed by \cite{polese2020experimental}, they deduce an empirical propagation loss model based on an extensive aerial measurement campaign. While, \cite{dabiri2020analytical} provides an tractable, closed-form statistical channel model for three types of UAV communication links: UAV-to-UAV and two types of relay links. They show that the performance of such links is largely dependent on the random movements of a UAV. \cite{zhang2019survey} gives a extensive overview on the different A2G and A2A channel models available in literature. An overview of potential spectrum management scenarios for mmWave enabled UAV swarm networks can be found in \cite{feng2018spectrum}, they propose a novel spectrum management architecture specifically for UAV-assisted cellular networks.

% \begin{itemize}
%     \item Use cases: BS, relay, backhauling, user
%     \item Integrated Access and Backhaul (IAB)
%     \item 3D beam-forming and beam-tracking \cite{song2020beam,zhang2019fast,yang2020performance}
%     \item Beam management \cite{kalamkar2020beam} \cite{meng20205g} is ML!
%     \item Mechanical and electrical tilting [5G-Sky]
%     \item Challenges of mmWave communication: wobbling, beam selection, handover, ...
%     \item Inter-UAV connectivity \cite{zhang2019fast,polese2020experimental,dabiri2020analytical}
%     \item TBD
% \end{itemize}


% \subsection{5G Multi-Segment Connectivity}


% \subsection*{Multi-Segment Integration in mmWave}

Literature: \cite{dabiri2020analytical}

==> OnePageIntro.tex <==
\section*{Short Introduction \\ \green{[Mahdi]}}


This study will focus on the followings:
\begin{itemize}
    \item Integrated ground-air-space communication and networking.
    \item 5G advancements and the road towards 6G and beyond. We aim to study solutions towards a fully connected segments for an ultimate goal of anytime, everywhere, and for everything services.
\end{itemize}

The weaknesses of each segment could be well covered by the strengths of the other segments for anytime, everywhere, and everything connectivity. 


Four challenges of wireless access networks [Halim]:
\begin{itemize}
    \item No connectivity in sparsely populated, rural, remote areas
    \item Poor connectivity in rural areas
    \item Pockets of poor ultra-connectivity in urban areas (permanent or temporary)
    \item Poor ultra-connectivity due to congestion (atypically high and unpredictable traffic demand)
\end{itemize}


Integrated ground-air-space is beneficial for the followings:
\begin{itemize}
    \item coverage in remote areas
    \item growth of data demand
    \item uneven data traffic
    \item emergency and disaster recovery
    \item rigid backbone networks
    \item flexible architecture for resource management and energy efficiency 
    \item dynamic network services such as dynamic edge computing and crowd sensing 
    \item significant reduction in the cost of deployment >> SpaceX
    \item increased demand for connectivity everywhere and anytime
\end{itemize}

Challenges ahead include:
\begin{itemize}
    \item Inherent super heterogeneity 
    \item Different constraints for different segments
    \item Intense co-channel interference and spectrum management
\end{itemize}

Key terms, ideas, and trending solutions to be aggregated and defined/described somewhere (maybe in the preliminary section):
\begin{itemize}
    \item beam hopping (BH)
    \item resource allocation
    \item Telemetry mining
\end{itemize}


Look at: 
https://www.linkedin.com/pulse/10-things-oq-technology-brings-help-you-use-5g-ntn-omar-qaise/?trackingId=ysgk6%2BooHAgmA8kCdZYQjA%3D%3D




1. footprint
2. spectrum availability and utilization
3. NT --> to be added to the table. also TN
4. all the ground-air-space to GAS
